Surface Agnostic Metrics for Cortical Volume Segmentation and Regression

The cerebral cortex performs higher-order brain functions and is thus implicated in a range of cognitive disorders. Current analysis of cortical variation is typically performed by fitting surface mesh models to inner and outer cortical boundaries and investigating metrics such as surface area and cortical curvature or thickness. These, however, take a long time to run, and are sensitive to motion and image and surface resolution, which can prohibit their use in clinical settings. In this paper, we instead propose a machine learning solution, training a novel architecture to predict cortical thickness and curvature metrics from T2 MRI images, while additionally returning metrics of prediction uncertainty. Our proposed model is tested on a clinical cohort (Down Syndrome) for which surface-based modelling often fails. Results suggest that deep convolutional neural networks are a viable option to predict cortical metrics across a range of brain development stages and pathologies.

==> paper2_results.tex <==
\section{Experimental Methods and Results}
\noindent\textbf{Data}: Data for this study comes from the Developing Human Connectome Project (dHCP) acquired in two stacks of 2D slices (in sagittal and axial planes) using a Turbo Spin Echo (TSE) sequence~\cite{Hughes2017ASystem}. The used parameters were: TR=12s, TE=156ms, SENSE factor 2.11 (axial) and 2.58 (sagittal) with overlapping slices. The study contains 505 subjects aged between 26-45 weeks. Tissue segmentations and surface metrics for training are derived form the dHCP surface extraction pipeline~\cite{Makropoulos2018TheReconstruction}\footnote{\href{https://github.com/BioMedIA/dhcp-structural-pipeline}{https://github.com/BioMedIA/dhcp-structural-pipeline}}.

A second clinical Down Syndrome cohort of 26 subjects was collected with a variety of scanning parameters, aged between 32-45 weeks, most subjects were acquired in the sagittal and transverse
planes using a multi-slice TSE sequence. Two stacks of 2D slices were acquired using the scanning parameters: TR=12s, TE=156ms, slice thickness = 1.6 mm with a slice overlap = 0.8 mm; flip angle = $90^{\circ}$ and an in-plane resolution: 0.8x0.8 mm.

\noindent\textbf{Preprocessing}: We project surface-based representations of cortical biometrics into a volumetric representation using a ribbon constrained method\footnote{\href{https://www.humanconnectome.org/software/workbench-command/-metric-to-volume-mapping}{https://www.humanconnectome.org/software/workbench-command/-metric-to-volume-mapping}} provided by the HCP project~\cite{Marcus2011InformaticsProject}. This operation is performed for both hemispheres of the brain and then combined into a single volume, where overlapping metric values are averaged. These volumes (together with the tissue segmentations) represent the training targets for the learning algorithm. T2w input volume and corresponding metric volumes are then resampled to a isotropic voxel spacing of 0.5 to ensure a prediction of physically meaningful values for each subject, \emph{i.e},  each voxel of our input image represents the same physical size in millimetres. Each T2 volume is intensity normalised to the range [0,1].

\noindent\textbf{Training}: 400 subjects are used for training; 50 for validation; 55 for test. During training we sample class-balanced 64x64x64 patches (N=12) from each subject's volume pair. We test on the entire volume of the image using a 3D sliding window approach. We conduct our experiments to predict two different cortical metrics: Thickness and Curvature.
\begin{figure}[h!]
\centering
    \begin{subfigure}[b]{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{gt_thick.png}
        \caption{Ground truth thickness map}
        \label{fig:dhcp_t_gt}
    \end{subfigure}
\hfill
    \begin{subfigure}[b]{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pred_thick.png}
        \caption{Predicted thickness map}
        \label{fig:dhcp_t_pred}
    \end{subfigure}
\hfill
    \begin{subfigure}[b]{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{diff_thick.png}
        \caption{Thickness difference Map}
        \label{fig:dhcp_t_diff}
    \end{subfigure}
\vfill
    \begin{subfigure}[b]{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{gt_curv.png}
        \caption{Ground truth curvature map}
        \label{fig:dhcp_c_gt}
    \end{subfigure}
\hfill
    \begin{subfigure}[b]{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pred_curv.png}
        \caption{Predicted curvature map}
        \label{fig:dhcp_c_pred}
    \end{subfigure}
\hfill
    \begin{subfigure}[b]{.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{diff_curv.png}
        \caption{Curvature difference Map}
        \label{fig:dhcp_c_diff}
    \end{subfigure}
\caption{Qualitative results on a dHCP subject: Here we have used ground truth surfaces to re-project our predicted metric volumes and difference map back into a surface representation for ease of comparison.}\label{fig:dhcp_qual}
\end{figure}

\begin{table}[h!]
\centering
\begin{tabular}{llll}
\multicolumn{1}{l|}{\textit{\textbf{Experiment}}} & \multicolumn{1}{l|}{Dice} & \multicolumn{1}{l|}{Mean error (mm)} & Median error (mm)\\ \hline
Thickness (mm) &  &  &\\ \hline
\multicolumn{1}{l|}{\textbf{UNetMSE}} & \multicolumn{1}{l|}{\textbf{0.946 $\pm$ 0.010}} &  \multicolumn{1}{l|}{\textbf{0.179 $\pm$ 0.025}} &  \textbf{0.125 $\pm$ 0.021} \\
\multicolumn{1}{l|}{UNetHuber} & \multicolumn{1}{l|}{0.939 $\pm$ 0.012} & \multicolumn{1}{l|}{0.197 $\pm$ 0.027} & 0.139 $\pm$ 0.022 \\ \hline
Curvature &  &  &\\ \hline
\multicolumn{1}{l|}{\textbf{UNetMSE}} & \multicolumn{1}{l|}{\textbf{0.945 $\pm$ 0.010}} & \multicolumn{1}{l|}{\textbf{0.0424 $\pm$ 0.005}} & \textbf{0.0304 $\pm$ 0.003}  \\
\multicolumn{1}{l|}{UNetHuber} & \multicolumn{1}{l|}{0.935 $\pm$ 0.011} & \multicolumn{1}{l|}{0.0498 $\pm$ 0.006} & 0.0361 $\pm$ 0.004 
\end{tabular}
\caption{Results for metric prediction: Metric error calculated as average voxel-wise difference between prediction and ground truth only for voxels within the cortex. Dice score is reported over the segmentation.}\label{tab:det_thick}
\end{table}

\noindent\textbf{Deterministic experiments}: We establish a baseline for simultaneous estimation of cortical segmentation and metric regression. Table~\ref{tab:det_thick} reports performance measures for all deterministic experiments. We find minimal difference in performance using the Huber loss function instead of MSE loss on the regression task module. Figure \ref{fig:dhcp_qual} show example outputs produced by our best performing model in comparison to the ground truth. Our network successfully extracts accurate cortical metric predictions directly from the input MRI, maintaining the structural variation we expect across the cortex. We notice that some extreme values have not been accurately predicted, such as in cortical regions at the bridge between the two brain hemispheres (for curvature prediction). However the extreme values that are present in the ground truth data are an artifact of the surface based metric prediction method, hence it is less important to replicate this precisely. In Figure~\ref{fig:downs_vio} we report test-set wide metrics comparing predicted global metric distributions in comparison to ground truth distributions, our method predicts a similar distribution of results to the ground truth.

\noindent\textbf{Probabilistic experiments}: We consider probabilistic extensions of our previous best performing method. Table \ref{tab:prob_table} reports performance measures for all probabilistic experiments. We find that introducing DropBlock layers into our network has improved segmentation accuracy, but metric estimation accuracy has declined. %However, further tuning of DropBlock parameters may improve performance above that of the deterministic approach. 
PHiSeg has not improved either segmentation or metric estimation performance. In these experiments, PHiSeg training was often unstable, and took much longer to converge than other methods. %Further training and tuning of PHiSeg parameters again may yield improved performance over deterministic measures.
While our error has increased, the ability to generate confidence maps for these predictions increases their value. Figure~\ref{fig:dhcp_conf} shows a generated confidence map using PHiSeg. % but as can be seen this is not the case, indicating further work is needed to improve the accuracy of our predictions.

\begin{table}[h!]
\centering
\begin{tabular}{lllll}
\multicolumn{1}{l|}{\textit{\textbf{Experiment}}} & \multicolumn{1}{l|}{Dice} & \multicolumn{1}{l|}{Mean Mean error} & \multicolumn{1}{l|}{Mean Median error} & Percent in range  \\ \hline
Thickness (mm) &  &  &\\ \hline
\multicolumn{1}{l|}{\textbf{UNetDropBlock}} & \multicolumn{1}{l|}{\textbf{0.945 $\pm$ 0.00}9} & \multicolumn{1}{l|}{\textbf{0.268 $\pm$ 0.017}} & \multicolumn{1}{l|}{\textbf{0.373 $\pm$ 0.017}} &  \textbf{59.83\%} \\
\multicolumn{1}{l|}{PHiSeg} & \multicolumn{1}{l|}{0.774 $\pm$ 0.075} & \multicolumn{1}{l|}{0.567 $\pm$ 0.096} & \multicolumn{1}{l|}{0.550 $\pm$ 0.052} & 19.60\%  \\ \hline
Curvature &  &  &\\ \hline
\multicolumn{1}{l|}{\textbf{UNetDropBlock}} & \multicolumn{1}{l|}{\textbf{0.946 $\pm$ 0.009}} & \multicolumn{1}{l|}{\textbf{0.0538 $\pm$ 0.004}} & \multicolumn{1}{l|}{\textbf{0.0705 $\pm$ 0.003}} & \textbf{56.19\%} \\
\multicolumn{1}{l|}{PHiSeg} & \multicolumn{1}{l|}{0.796 $\pm$ 0.022} & \multicolumn{1}{l|}{0.102 $\pm$ 0.006} &  \multicolumn{1}{l|}{0.102$\pm$ 0.006} & 24.98\%
\end{tabular}
\caption{Probabilistic Prediction results: We show dice scores and the mean metric error when taking mean and the median of multiple (N=5) predictions as the final output.}\label{tab:prob_table}
\end{table}
%\textbf{\textit{Confidence maps vs diff}}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{curv_conf_phi.png}
    \caption{Confidence map generated with PHiSeg for a dHCP subject. Brighter areas indicate decreased confidence. }
    \label{fig:dhcp_conf}
\end{figure}

\noindent{\textbf{Down Syndrome experiments}}: We assess the performance of our method on a challenging Down Syndrome MRI dataset for which the dHCP pipeline fails to extract metrics correctly for many subjects. Since the 'ground truth' for this dataset is error prone, we demonstrate the performance of our method qualitatively and through population comparisons to the healthy dHCP test set used in previous experiments. Figure~\ref{fig:downs_surf} shows that our method produces more reasonable estimates of cortical thickness than the dHCP pipeline, thus showing evidence for our method's robustness to challenging datasets. Population statistics indicating that our method produces metric values in a sensible range for cortical thickness are shown in Figure~\ref{fig:downs_vio}. However our predicted distribution for cortical curvature is not consistent with healthy patients, indicating curvature and other more complex metrics remain challenging.
%, not dissimilar from healthy patients. 

\begin{figure}[h!]
\centering
    \begin{subfigure}[b]{.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{gt_thick_d.png}
        \caption{}
    \end{subfigure}
\hfill
    \begin{subfigure}[b]{.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pred_thick_d.png}
        \caption{}
    \end{subfigure}
\vfill
    \begin{subfigure}[b]{.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{gt_curv_d.png}
        \caption{}
    \end{subfigure}
\hfill
    \begin{subfigure}[b]{.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pred_curv_d.png}
        \caption{}
    \end{subfigure}
    \caption{Qualitative results on Down Syndrome dataset: a) dHCP predicted thickness; b) Our method predicted thickness; c) dHCP predicted curvature; d) Our method predicted curvature.}\label{fig:downs_surf}
\end{figure}

\begin{figure}[h!]
\centering
    \begin{subfigure}[b]{.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{dhcp_thickness_violin.pdf}
        \caption{Thickness distributions}
        \label{fig:thick_vio}
    \end{subfigure}
% \hfill
    \begin{subfigure}[b]{.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{dhcp_curvature_violin.pdf}
        \caption{Curvature distributions}
        \label{fig:curv_vio}
    \end{subfigure}
    \caption{Global average metric distributions a) Thickness and b) Curvature. Our method produces a sensible distribution of values for the Down Syndrome data set compared to the dHCP pipeline for thickness prediction. However curvature prediction remains challenging. Pathological cases (right two in each plot) cannot be quantitatively evaluated because of missing ground truth.}\label{fig:downs_vio}
\end{figure}

